On scalable and efficient training of diffusion samplers

We address the challenge of training diffusion models to sample from unnormalized energy distributions in the absence of data, the so-called diffusion samplers. Although these approaches have shown promise, they struggle to scale in more demanding scenarios where energy evaluations are expensive and the sampling space is high-dimensional. To address this limitation, we propose a scalable and sample-efficient framework that properly harmonizes the powerful classical sampling method and the diffusion sampler. Specifically, we utilize Monte Carlo Markov chain (MCMC) samplers with a novelty-based auxiliary energy as a Searcher to collect off-policy samples, using an auxiliary energy function to compensate for exploring modes the diffusion sampler rarely visits. These off-policy samples are then combined with on-policy data to train the diffusion sampler, thereby expanding its coverage of the energy landscape. Furthermore, we identify primacy bias, i.e., the preference of samplers for early experience during training, as the main cause of mode collapse during training, and introduce a periodic re-initialization trick to resolve this issue. Our method significantly improves sample efficiency on standard benchmarks for diffusion samplers and also excels at higher-dimensional problems and real-world molecular conformer generation.

==> math_commands.tex <==
% auto-generated wrapper to satisfy \input{math_commands}
% This file tells LaTeX to load the style file math_commands.sty
\RequirePackage{math_commands}

==> resources/figures/aldp_histograms.tex <==
% \begin{figure}[t]
%     \centering

%     % ALDP Energy Histogram
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=0.5\linewidth]{resources/images/aldp_energy_hist.pdf}
%     \end{subfigure}
%     \hfill
%     % ALDP Interatomic Distance Histogram
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=0.5\linewidth]{resources/images/aldp_interatomic_distances.pdf}
%     \end{subfigure}

%     \caption{\textbf{Distributions of energy and interatomic distance for Alanine Dipeptide.}}
%     \label{fig:aldp_histograms}
% \end{figure}

\begin{wrapfigure}{r}{0.4\textwidth}  % 오른쪽 정렬, 너비는 텍스트 너비의 40%
  \centering
  % 에너지 히스토그램
  \includegraphics[width=\linewidth,height=0.5\linewidth]{resources/images/aldp_energy_hist.pdf}
  \caption{\textbf{Distribution of energy for Alanine Dipeptide.}}
  \label{fig:aldp_energy_histogram}
\end{wrapfigure}



==> resources/figures/aldp_ramachandran.tex <==
% \begin{figure}[t]
%     \centering
%     % 6 subfigures in one row (Ground Truth and Ours first)
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/gt_phi_psi.png}
%         \caption{Ground Truth}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/ours_phi_psi_2.png}
%         \caption{Ours}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/tb_expl_ls_phi_psi.png}
%         \caption{TB+Expl+LS}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/pis_phi_psi.png}
%         \caption{PIS}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/mle_phi_psi.png}
%         \caption{MLE}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{example-image-duck}
%         \caption{FAB}
%     \end{subfigure}

%     \caption{
%         \textbf{Ramachandran plot of Alanine Dipeptide}.
%     }
%     \label{fig:aldp_ramachandran_plot}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{resources/images/phi_psi.pdf}
    \caption{
        \textbf{Ramachandran plot of Alanine Dipeptide.}
    }
    \label{fig:aldp_ramachandran_plot}
\end{figure}

==> resources/figures/aldp_visualization.tex <==
% \begin{figure}[t]
%     \centering
%     % 6 subfigures in one row (Ground Truth and Ours first)
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/aldp_3d_gt.png}
%         \caption{Ground Truth}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/aldp_3d_ours.png}
%         \caption{Ours}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/aldp_3d_tb_expl_ls.png}
%         \caption{TB+Expl+LS}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/aldp_3d_pis.png}
%         \caption{PIS}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{resources/images/aldp_3d_mle.png}
%         \caption{MLE}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth,height=\linewidth]{example-image-duck}
%         \caption{FAB}
%     \end{subfigure}

%     \caption{
%         \textbf{3D visualization of sampled conformation of Alanine Dipeptide.}
%     }
%     \label{fig:aldp_visualization}
% \end{figure}


\begin{figure}[t]
    \vspace*{-0.5cm}    
    \centering
    \includegraphics[width=0.7\textwidth]{resources/images/3d_visualization.pdf}
    \caption{
        \textbf{3D visualization of sampled conformation of Alanine Dipeptide.}
    }
    \label{fig:aldp_visualization}
    \vspace{-0.5cm}
\end{figure}

==> resources/figures/tri_tetra.tex <==
% \begin{figure*}[t]
%   \centering
%   %--- (a) Dipeptide, tripeptide, tetrapeptide Table
%   \begin{subfigure}{0.6\textwidth}
%     %\centering
%     %\vspace{0pt}  
%     %\renewcommand{\arraystretch}{1.2}
%     \resizebox{\linewidth}{!}{
%       \begin{tabular}{l c c c}
%         \toprule
%         \textbf{Method} & Dipeptide & Tripeptide & Tetrepeptide \\
%         \midrule
%         MLE (1M) & $17.414 \pm 0.142$ & $6.117 \pm 0.019$ & $29.072 \pm 0.560$ \\
%         \emph{SGDS} (1M) & $\mathbf{17.109 \pm 0.165}$ & $\mathbf{5.600 \pm 0.030}$ & $\mathbf{26.600 \pm 0.214}$ \\
%         \bottomrule
%       \end{tabular}
%     }
%     \vspace{.2in}
%     \caption{EUBO-ELBO gaps on peptides}
%     \label{tab:peptides_table}
%   \end{subfigure}
%   % \hfill
%   %--- (b) tripeptide, tetrapeptide visualizations
%   \begin{subfigure}{0.39\textwidth}
%     \centering
%     % \includegraphics[width=\linewidth]{resources/images/lj55_trade_off.pdf}
%     \includegraphics[width=\linewidth]{resources/images/tri_tetra_3d_visualization.png}
%     \caption{3D visualization of tri- and tetrapeptides}
%     \label{fig:tri_tetra_visualization}
%   \end{subfigure}
%   \label{fig:tri_tetra_peptide}
% \end{figure*}

==> resources/tables/ablation.tex <==
\begin{table*}[t]
\caption{Ablation study comparing ELBO, ELBO\_RW, and EUBO under different strategies with 20M energy calls. The target distribution is Manywell 128.}
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{6pt}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{l c c}
\toprule
\textbf{Method} & ELBO $\uparrow$ & EUBO $\downarrow$\\
\midrule
AIS+MLE               & $244.85 \pm 10.34$ & $840.45 \pm 11.59$ \\
Fine-tuning           & $554.17 \pm 107.70$ & $707.07 \pm 8.49$ \\
Re-init w/o log $Z$   & $583.65 \pm 16.69$ & $691.37 \pm 1.40$ \\
w/o RND-searcher   & $608.01 \pm 4.18$ & $686.63 \pm 1.32$ \\
\midrule
\emph{SGDS} & $\mathbf{614.41 \pm 3.44}$ & $\mathbf{684.76 \pm 1.30}$ \\
\bottomrule
\end{tabular}
 }
\label{tab:ablation}
\end{table*}


==> resources/tables/peptides_table.tex <==
\begin{tabular}{l c c}
\toprule
\textbf{Method} & ELBO $\uparrow$ & EUBO $\downarrow$\\
\midrule
AIS+MLE               & $244.85 \pm 10.34$ & $840.45 \pm 11.59$ \\
Fine-tuning           & $554.17 \pm 107.70$ & $707.07 \pm 8.49$ \\
Re-init w/o log $Z$   & $583.65 \pm 16.69$ & $691.37 \pm 1.40$ \\
w/o RND-searcher   & $608.01 \pm 4.18$ & $686.63 \pm 1.32$ \\
\midrule
\emph{SGDS} & $\mathbf{614.41 \pm 3.44}$ & $\mathbf{684.76 \pm 1.30}$ \\
\bottomrule
\end{tabular}
 }
\label{tab:peptide_table}
\end{table*}
